Toward Less Hidden Cost of Code Completion with Acceptance and Ranking Models

Code completion is widely used by software developers to provide coding suggestions given a partially written code snippet. Apart from the traditional code completion methods, which only support single token completion at minimal positions, recent studies show the ability to provide longer code completion at more flexible positions. However, such frequently triggered and longer completion results reduce the overall precision as they generate more invalid results. Moreover, different studies are mostly incompatible with each other. Thus, it is vital to develop an ensemble framework that can combine results from multiple models to draw merits and offset defects of each model. This paper conducts a coding simulation to collect data from code context and different code completion models and then apply the data in two tasks. First, we introduce an acceptance model which can dynamically control whether to display completion results to the developer. It uses simulation features to predict whether correct results exist in the output of these models. Our best model reduces the percentage of false-positive completion from 55.09% to 17.44%. Second, we design a fusion ranking scheme that can automatically identify the priority of the completion results and reorder the candidates from multiple code completion models. This scheme is flexible in dealing with various models, regardless of the type or the length of their completion results. We integrate this ranking scheme with two frequency models and a GPT-2 styled language model, along with the acceptance model to yield 27.80% and 37.64% increase in TOP1 and TOP5 accuracy, respectively. In addition, we propose a new code completion evaluation metric, Benefit-Cost Ratio(BCR), taking into account the benefit of keystrokes saving and hidden cost of completion list browsing, which is closer to real coder experience scenario.

==> gpt2.tex <==
\section{GPT-2 setup} 

GPT-2, as a an auto-regressive pre-train language model, has demonstrate its strong ability in both text and code generation area. It consists of a multi-layer transformer decoder stack, which maps input tokens' embedding and positions' embedding into an raw output hidden-state, followed by a linear layer to calculate prediction score for each vocabulary token. We train our GPT-2 model from scratch with source code data.

\subsection{Model structure}

Considering the trade-off between accuracy and performance, we select small GPT-2 124M model and apply minor modification to build our GPT-2 model for the code completion task. The maximum sequence length is reduced from 1024 to 256 and the vocabulary size is reduced from 50257 to 30000. Final model hyper-parameters are shown in Table \ref{tab:GPT_paras}. Our final GPT-2 model has 108M parameters.

\begin{table}[h]
  \caption{GPT-2 model architecture hyper-parameters}
  \label{tab:GPT_paras}
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lll}
    \toprule
    Hyper-parameter & Explanation & Value\\
    \midrule
    n\_layer & Number of transformer layers & 12\\
    n\_model & Dimension of hidden states & 768\\
    n\_embd & Dimension of embedding & 768\\
    n\_head & Number of attention heads & 12\\
    n\_positions & Max code token length & 256\\
    p\_drop & Drop probability & 0.1\\
    vocab\_size & Vocabulary size & 30000\\
  \bottomrule
\end{tabular}}
\end{table}

\subsection{Preprocessing}

We apply following preprocessing steps to the source code, including:
\begin{itemize}
  \item Partially remove comments: 
  Original source code has several kinds of comments, some of them might inspire GPT2 model to  predict correct results even these tokens are unseen in the input code tokens. In general, we only keep pure comment lines before the function definition and docstrings below the function definition, since they are normally the description of the current function. 
  \item remove non-English letters and symbols: 
  The source code hosted on internet code platform such as Github are contributed by coders from different countries. Thus, the source code might consist of multilingual tokens. To avoid garbled output and maintain standardized code generation, we only keep the English letters and symbols in the training and test source code.
  \item Replace long string/number with special placeholder: 
  Coder might unintentionally leave irrelevant and potentially sensitive information in string or number literals within their code projects. On the other hand, some frequently used string literals, such as "\_\_main\_\_", "default", "GET", can be seen as keywords and directly used in the completion. Thus, We set two thresholds, frequency of occurrence and literal length, as criterion to decide whether the string/number literals should be replaced as a special placeholder in the source code.
\end{itemize}

\subsection{Tokenizer}

Tokenizer is used to encode source code into a sequence of tokens prior to feeding into GPT2 model, and decode model output back to a code literal. We use the same tokenization method, Byte-Pair Encoding (BPE), with the original GPT2 model. It is a unsupervised tokenizer, which recursively replaces most frequently occurring pair of Unicode characters with a new character in the vocabulary. We retrain BPE tokenizer from scratch using our source code data and set the vocabulary size as 30000.   

\subsection{Inference}

We apply beam-search method in GPT2 inference procedure to generate code completion result. Beam-search reduces the risk of missing hidden high probability token sequences by keeping the top k (k is the beam size) aggregate highest probability sequences at each step. In order to reduce the redundant calculation and accelerate the inference during the beam-search, we adjust the beam size dynamically at each step by setting the following criterion:
\begin{itemize}
  \item terminate the output sequence if its aggregate score lower than a score threshold t. 
  \item terminate the output sequence if it has end-of-line token ('$\backslash$n').
  \item terminate the output sequence if it has a annotation symbol.
  \item terminate the output sequence if it runs into closed loop.
  \item terminate the output sequence if it reaches the maximum inference steps.
\end{itemize}

Figure \ref{fig:beam_search} illustrates one of our beam-search example with beam size k and score threshold t being set as 5 and -3 respectively. At the step 1, top 5 score candidates are selected and combined as a batch for the step 2 inference. At the step 2, we also take top 5 candidates with highest aggregate score, in which only two candidates have aggregate score higher than the threshold t. Thus, only 2 candidates are selected for the next step inference, which means the batch size of step 3 input is 2. The rest inference steps can be done in the same manner until our criterion terminate all beam. Thus, instead of doing beam-search with fixed batch size inference at each step, we dynamically adjust the batch size according to the previous step result. In this case (Figure \ref{fig:beam_search}), we reduce the calculation cost from (batch size 5 * 10 steps) in naive beam-search to (batch size 5 * 1 step + batch size 2 * 9 steps). 

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{images/beam-search.PNG}
  \caption{GPT-2 beam-search}
  \Description{}
  \label{fig:beam_search}
\end{figure*}





